Supersymmetry and the Spectral Action. On a geometrical interpretation of the MSSM

This PhD thesis aims at combining the framework of noncommutative geometry and supersymmetry. A particular class of non-commutative geometries called almost-commutative geometries can be used to describe particle theories. This thesis contains a systematic search for such almost-commutative geometries whose corresponding spectral action exhibits supersymmetry. Chapter 2 discusses extensions of the Standard Model in the context of noncommutative geometry in general. In Chapter three a framework is developed to build and analyze potential supersymmetric theories. Chapter 4 covers supersymmetry breaking mechanisms in this context. Finally, the approach of Chapter three is applied to what is to yield the non-commutative version of the MSSM in Chapter 5.

==> Chapters/CV.tex <==

	\input{FrontBackmatter/CV}


==> Chapters/Summary/Samenvatting.tex <==
\selectlanguage{dutch}
\section{Samenvatting}

Al vele eeuwen probeert de mens de wereld om hem heen te \emph{begrijpen}, in te bedden in logische structuren, patronen en wetmatigheden te ontwaren in de ogenschijnlijke chaos om ons heen. Dit noemen we wetenschap. In de natuurkunde spitsen we ons grosso modo toe op de `dode' natuur; hoe fysieke objecten bewegen, met elkaar interageren en waaruit ze bestaan. Die laatste vraag vormt feitelijk de basis van mijn vakgebied, de hoge-energie fysica, maar daarover later meer. De manier waarop we dat doen is in wezen redelijk simpel; we formuleren een bepaalde hypothese en testen vervolgens met behulp van experimenten of en in hoeverre die hypothese klopt. De taal waarin die hypotheses in de natuurkunde typische geformuleerd worden, is die van de wiskunde. Dat heeft goede redenen, want de wiskunde stelt ons in staat om heel precieze hypotheses op te stellen: een uitspraak als
\begin{quote}
	``bla ''
\end{quote}
is namelijk een stuk nauwkeuriger dan 
\begin{quote}
	``hoe harder je tegen een bal aanschopt, hoe harder deze zich van je afbeweegt''.
\end{quote}
Dit onderscheid is van essentieel belang, want hoe nauwkeuriger de uitspraak is die een wetenschapper maakt, hoe makkelijker het voor elke andere wetenschapper is om te bepalen of deze het met de uitspraak eens is. Een wetenschappelijke theorie is in essentie een aantal samenhangende uitspraken over hoe de natuur zich gedraagt, of zou moeten gedragen. In de loop van de tijd hebben we steeds betere apparatuur weten te ontwikkelen om onze hypotheses te testen en als gevolg daarvan hebben we steeds betere theorie\"en weten te ontwikkelen. Met `beter' bedoel ik hier niet alleen `nauwkeuriger' maar ook toepasbaar op steeds meer situaties. Sinds Isaac Newton (1642 - 1727) weten we bijvoorbeeld dat de wetmatigheid die ten grondslag ligt aan een pen die je laat vallen, precies dezelfde is als die de planeten in hun baan om de zon houdt. Dat is nog eens een veralgemenisering! \\

De heilige graal van de natuurkunde is dan ook om \'e\'en fundamentele theorie te formuleren waarmee we uiteindelijk \'alle situaties kunnen beschrijven ---en dus begrijpen--- die wij experimenteel kunnen toetsen. Historisch gezien betekende dat vaak dat aan een theorie die goed werkte in een bepaalde situatie, achteraf een \'andere theorie ten grondslag lag die breder toepasbaar is maar waaruit we de oorspronkelijke theorie kunnen herleiden door toe te spitsen op de situatie waarin deze goed werkte. Dat klinkt nogal abstract, dus laat ik een voorbeeld geven. Tot ruim een eeuw geleden wisten we niet beter dan dat de wereld perfect te beschrijven is met behulp van de Newtonse mechanica; $F = m \times a$, actie = reactie, enzovoort. Echter, Einstein leerde ons in 1905 dat dit niet meer het geval is bij hele hoge snelheden, snelheden die in de buurt komen van de lichtsnelheid. Is de mechanica van Newton daarmee fout? Nee, we weten alleen dat haar toepasbaarheid beperkt is tot relatief lage snelheden, en dat we voor hogere snelheden rekening moeten houden met de eindigheid van de lichtsnelheid. Dit gegeven heeft Einstein geleid tot zijn de Speciale Relativiteitstheorie.\\

De lichtsnelheid is een \emph{fundamentele natuurconstante} gebleken, welke dezelfde waarde heeft waar en wanneer we deze ook mogen meten. Zo springen er nog twee constantes uit die van soortgelijk belang zijn. De ene geeft aan of er zwaartekracht in het spel is of niet, de andere over hoe groot de objecten zijn die we bestuderen. Zouden we nu een theorie vinden die de wereld nauwkeurig beschrijft voor zowel willekeurig hoge snelheden, als voor willekeurige kleine afmetingen, als voor willekeurig sterke zwaartekracht, dan kunnen we natuurkunde-afdelingen wereldwijd sluiten. De Figuur \ref{fig:intro_theory_cube} in de inleiding van dit proefschrift is een grafische weergave van bovenstaande; we zijn op zoek naar een theorie (`QG') die correspondeert met de bovenste hoek vooraan de kubus, vanwaar we naar alle andere andere hoeken (theorie\"en) kunnen lopen die hieruit voortvloeien voor specifiekere situaties, zoals bij lage snelheden, voor grotere afmetingen of voor een zwakkere zwaartekracht. \\

Het specifieke wetenschapsgebied waar ik in gewerkt heb, stelt zich de vraag wat nu eigenlijk de fundamentele bouwstenen van de wereld om ons heen zijn. De tafel waaraan we zitten, de vork waarmee we eten en het glas waaruit we drinken; waar zijn die van gemaakt? Hout, staal en glas, zou je op het eerste gezicht zeggen, maar hoe verschilend zijn deze materialen? Door ze goed te bestuderen hebben we bouwstenen weten te identificeren waaruit allen gemaakt zijn: atomen. Hout bestaat voornamelijk uit koolstof-atomen, in staal zitten hoofdzakelijk ijzer-atomen en in glas komen silicium-atomen veelvuldig voor. We hebben een flink aantal types van dergelijke atomen, 118 om precies te zijn. Omdat die atomen zo klein zijn, schiet de Newtonse mechanica schromelijk tekort om atomen te begrijpen; we moeten ons hiervoor wenden tot de quantum mechanica. Lang dachten we dat deze atomen de kleinste bouwstenen waren. Inmiddels weten we beter; al deze atomen blijken te bestaan uit kernen van protonen en neutronen waaromheen \'e\'en of meer elektronen `cirkelen'. Van die elektronen denken we tot op de dag van vandaag nog steeds dat ze ondeelbaar zijn, maar de protonen en neutronen blijken op hun beurt weer uit zogenoemde `up-quarks' en `down-quarks' te bestaan. Inmiddels zijn de deeltjes waarover we het hebben z\'o klein geworden, dat zelfs de quantum mechanica niet meer afdoende is om ze te begrijpen. De kwantumveldentheorie is de theorie die niet alleen met hele kleine afmetingen overweg kan, maar ook met heel hoge snelheden. Deze kwantumveldentheorie is extreem succesvol; deze goed snappen heeft ons in staat gesteld om te beschrijven welke elementaire deeltjes\footnote{We noemen een deeltje `elementair' als we nog geen reden hebben om aan te nemen dat deze op zijn beurt weer uit nog kleinere bouwstenen bestaat.} er zijn, en hoe ze met elkaar interageren. Zo hebben we al het electron en het up- en down-quark gezien. Je kunt je afvragen waarom die deeltjes bij elkaar blijven zitten in een atom; er is toch niets dat ze tegenhoudt hun eigen weg te gaan? Het blijkt dat er ook zogenoemde krachtoverdragende deeltjes zijn. Doordat de electronen en quarks dergelijke deeltjes `uitwisselen' worden ze tot elkaar aangetrokken, of van elkaar afgestoten. Dit zorgt ervoor dat de quarks netjes in de protonen en neutronen blijven zitten, de elektronen daar omheen blijven cirkelen en uiteindelijk dat er \"uberhaupt zoiets kan bestaan als een tafel om aan te zitten, een vork om mee te eten en een glas om uit te drinken.\\

 Het plaatje blijkt hier nog niet mee compleet; van het elekton en de twee quarks blijken nog twee bijna identieke kopie\"en te zijn. Daarvan krijgen wij op aarde bijzonder weinig mee, maar uit onderzoek met deeltjesversnellers en andere experimenten weten we dat ze er weldegelijk zijn. Daarbovenop kwam men er in de jaren 60 van de vorige eeuw achter dat de theorie van al die deeltjes alleen maar kloppend kan zijn wanneer er n\'og een type deeltje was, eentje waarvoor op dat moment experimenteel gezien nog geen enkele aanleiding was. En inderdaad, in 2012 werd dit zogenoemde Higgs-deeltje\footnote{Ere wie ere toekomt: eigenlijk moeten we spreken over het Brout-Englert-Higgs-Guralnik-Kibble-Hagen-deeltje, maar dat bekt niet zo lekker.} experimenteel aangetoond, wat het sluitstuk vormde voor wat we het Standaard Model zijn gaan noemen. In Figuur \ref{fig:SM-simplified} staat een schematisch overzicht van dat Standaard Model afgebeeld. Deze theorie is zo succesvol, dat het vooralsnog zelfs de testen van krachtigste deeltjesversnellers op aarde weerstaat! \\

\begin{figure}[h]
	\centering
		\def\svgwidth{\textwidth}
		\includesvg{SM_simplified}
		\caption{Alle deeltjes van het standaard model; materiedeeltjes zijn weergegeven met rondjes, en krachtoverdragende deeltjes zijn aangegeven met lijntjes. Als er een lijntje staat tussen twee rondjes betekent dit dat de deeltjes die door de rondjes voorgesteld worden de krachtdeeltjes uitwisselen die horen bij het betreffende lijntje. De letter $u$ staat voor up-quark, $d$ voor down-quark, $e$ voor elektron en $\nu$ voor neutrino. We hebben de volgende krachtoverdragende deeltjes: het foton $\gamma$, de dragers van de zwakke kernkracht $W^+, W^-$ en $Z^0$ en tenslotte de dragers van de sterke kernkracht $g$. Dit diagram is een flinke versimpeling van het complete plaatje; sommige van de krachtoverdragende deeltjes (de lijntjes), bijvoorbeeld, interageren ook weer met elkaar of met zichzelf.}
		\label{fig:SM-simplified}
\end{figure}

Betekent dit dan de gevreesde sluiting van alle faculteiten natuurkunde? Geenszins, er zijn nog tal van open vragen en niet opgeloste problemen.





==> Chapters/Summary/Summary.tex <==
\selectlanguage{american}
\section{Summary}



==> FrontBackmatter/Colophon.tex <==
\pagestyle{empty}

\hfill

\vfill


\pdfbookmark[0]{Colophon}{colophon}
\section*{Colophon}
This document was typeset using the typographical look-and-feel \texttt{classicthesis} developed by Andr\'e Miede. 
The style was inspired by Robert Bringhurst's seminal book on typography ``\emph{The Elements of Typographic Style}''. 
\texttt{classicthesis} is available for both \LaTeX\ and \mLyX: 
\begin{center}
\url{http://code.google.com/p/classicthesis/}
\end{center}
Happy users of \texttt{classicthesis} usually send a real postcard to the author, a collection of postcards received so far is featured here: 
\begin{center}
\url{http://postcards.miede.de/}
\end{center}
 
\bigskip

\noindent\finalVersionString

%Hermann Zapf's \emph{Palatino} and \emph{Euler} type faces (Type~1 PostScript fonts \emph{URW
%Palladio L} and \emph{FPL}) are used. The ``typewriter'' text is typeset in \emph{Bera Mono}, 
%originally developed by Bitstream, Inc. as ``Bitstream Vera''. (Type~1 PostScript fonts were made 
%available by Malte Rosenau and
%Ulrich Dirr.)

%\paragraph{note:} The custom size of the textblock was calculated
%using the directions given by Mr. Bringhurst (pages 26--29 and
%175/176). 10~pt Palatino needs  133.21~pt for the string
%``abcdefghijklmnopqrstuvwxyz''. This yields a good line length between
%24--26~pc (288--312~pt). Using a ``\emph{double square textblock}''
%with a 1:2 ratio this results in a textblock of 312:624~pt (which
%includes the headline in this design). A good alternative would be the
%``\emph{golden section textblock}'' with a ratio of 1:1.62, here
%312:505.44~pt. For comparison, \texttt{DIV9} of the \texttt{typearea}
%package results in a line length of 389~pt (32.4~pc), which is by far
%too long. However, this information will only be of interest for
%hardcore pseudo-typographers like me.%
%
%To make your own calculations, use the following commands and look up
%the corresponding lengths in the book:
%\begin{verbatim}
%    \settowidth{\abcd}{abcdefghijklmnopqrstuvwxyz}
%    \the\abcd\ % prints the value of the length
%\end{verbatim}
%Please see the file \texttt{classicthesis.sty} for some precalculated 
%values for Palatino and Minion.
%
%    \settowidth{\abcd}{abcdefghijklmnopqrstuvwxyz}
%    \the\abcd\ % prints the value of the length






==> FrontBackmatter/Dedication.tex <==
%*******************************************************
% Dedication
%*******************************************************
\thispagestyle{empty}
%\phantomsection 
\refstepcounter{dummy}
\pdfbookmark[1]{Dedication}{Dedication}

\vspace*{3cm}


\begin{flushright}
	In loving memory of Cees --Opie-- van den Broek (1921 -- 2013)
\end{flushright}

%\begin{center}
\begin{flushright}
Have you ever heard about the Higgs Boson blues?\\
I'm goin' down to Geneva baby, gonna teach it to you.\\\medskip
	--- Nick Cave 
\end{flushright}
%\end{center}


==> FrontBackmatter/DirtyTitlepage.tex <==
%*******************************************************
% Little Dirty Titlepage
%*******************************************************
\thispagestyle{empty}
%\pdfbookmark[1]{Titel}{title}
%*******************************************************
\begin{center}
    \spacedlowsmallcaps{\myName} \\ \medskip                        

    \begingroup
        \color{Maroon}\spacedallcaps{\myTitle}
    \endgroup
\end{center}        


==> FrontBackmatter/Publication.tex <==
%*******************************************************
% Publications
%*******************************************************
\pdfbookmark[1]{Publications}{publications}
\chapter*{Publications}

\begin{thebibliography}{91}
 \providecommand{\natexlab}[1]{#1}
 \providecommand{\url}[1]{\texttt{#1}}
 \expandafter\ifx\csname urlstyle\endcsname\relax
   \providecommand{\doi}[1]{doi: #1}\else
   \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi
 
 \bibitem[Alvarez et~al.(1995)Alvarez, Gracia-Bond\'ia, and
   Mart\'in]{Alvarez1995}
 E.~Alvarez, J.M. Gracia-Bond\'ia, and C.P. Mart\'in.
 \newblock Anomaly cancellation and gauge group of the standard model in {NCG}.
 \newblock \emph{Phys. Lett. B}, 364:\penalty0 33--40, 1995.
\end{thebibliography}




The contents of this thesis are based on the following publications:
%Some ideas and figures have appeared previously in the following publications:
%\begin{itemize}

%\begin{thebibliography}{99}
%	\item Chapter \ref{ch:constraints} is based on \bibitem{BS12}.
%\end{thebibliography}
%
%\begin{itemize}	
%	\item Chapter \ref{ch:sst} is based on \cite{BS14I}.
%
%	\item Chapter \ref{ch:breaking} is based on \cite{BS14II}.
%
%	\item Chapter \ref{ch:NCMSSM} is based on \cite{BS14II}.
%\end{itemize}

\bigskip


==> FrontBackmatter/Titlepage.tex <==
%*******************************************************
% Titlepage
%*******************************************************
\begin{titlepage}
	% if you want the titlepage to be centered, uncomment and fine-tune the line below (KOMA classes environment)
	\begin{addmargin}[-1cm]{-3cm}
    \begin{center}
        \large  

        \hfill

        \vfill

        \begingroup
            \color{Maroon}\spacedallcaps{\myTitle} \\ \bigskip
        \endgroup

        \spacedlowsmallcaps{\myName}

        \vfill

      %  \includegraphics[width=6cm]{gfx/TFZsuperellipse_bw} \\ \medskip

        \mySubtitle \\ \medskip   
        %\myDegree \\
        %\myDepartment \\                            
        %\myFaculty \\
        %\myUni \\ \bigskip

        \myTime

        \vfill                      

    \end{center}  
  \end{addmargin}       
\end{titlepage}   


==> FrontBackmatter/acknowledgements.tex <==

\chapter{Acknowledgements}

% Begeleiders --> Walter Wim, Ronald.

% oud-collega's --> Harm, Marcel, Stefan G, Stefan J, Magda, Melvin, Folkert, Yiannis, GJ, Vince, Antonia, Antonio, Gijs, Irene, Jose, Guus, Jins, Jari, Margot, secretariaat, en alle anderen, HEF master students of any generation. 

% GroenLinks --> Pepijn O., Wouter, Cilia, Nynke, Louis, Giedo, Joep, Lisa, April, Marieke

% Zwammen --> Frank, Kimberly, Anco, Koen, Maaike, Maarten

% TPP-group --> Jan, Wilco, Jordy, Sander, Jacob, Pablo, Reinier, Rob, Lisa, (Tiago, Keri, Chiara, Giuseppe, Ivano)

Trainingsbureau --> Eline, Anouk, Sascha, ...

% Fietsen --> Youri, LJ, Jeroen, Vincent, Bas L.

% Banenrepubliek --> Matthijs, Galina, Jonas

Overige --> B&F, CB, Floris, Hans, Geerten & Patricia

(schoon)Familie

Petra

First of all I would like to thank my advisor Ronald Kleiss, and both of my supervisors Wim Beenakker and Walter van Suijlekom, in the first place for having loads of patience with me, for being open for discussion anytime and stimulating me to keep on pushing the envelope. You are not the only ones that made the HEP department such a great place to work at, though. The secretariat was a welcome place anytime, every time. Thank you Marjo, Gemma and Annelies. Admittedly, the atmosphere at the department was one of the reasons to choose this job. At many times it was more of a group of friends than an office. Many people deserve to be thanked for that. Antonia, Antonio, Ben, Folkert, Gijs, GJ, Guus, Harm, Irene, Jos\'e, Jari, Jins, Koen, Magda, Margot, Marcel, Matthias, Melvin, Stefan J, Stefan G, Vince, Yiannis and many other (you know who you are). You are the best, I've had wonderful times with you during but even more so after work. Thanks a million for making the time at the department what it was. 

Being part of the TPP-programme taught me that there are cool physicists outside of the province as well. Chiara, Ivano, Jacob, Jan, Jordy, Lisa, Pablo, Reinier, Rob, Sander, Tiago, Wilco and again many more. I enjoyed the Fridays at Nikhef and the school in Driebergen almost as much as going to the Ij-brouwerij, the Opposites concert and Brazil. Thank you.

But honestly, I doubt whether I would have coped doing a PhD if it wasn't for all those great and valuable things to keep it in balance with. The `zwammen'-group for instance, with Anco, Frank, Kimberly, Koen, Maaike and Maarten. Whether we were having the serious conversations that have broadened my academic perspective, or the lighter ones, I enjoyed them equally well.

The guys and girl from the Banenrepubliek, Matthijs, Galina and Jonas (and the rest that I have mentioned previously already): regrettably we were maybe too successful, but it was a good and stimulating initiative nonetheless.

The AKKU trainingsbureau, ...

From doing all that mental labour one craves for some physical exercise once in a while. Luckily I was surrounded with many people that like to do cycling as well. Whether it was done in the vicinity of Nijmegen, on one of the NFC-weekends of even somewhere high up in the Alps, it was always fun to do. Thank you Youri, LJ, Jeroen, Vincent, and Bas.

Then there are the people from GroenLinks. It always felt like a family when I was with you. Making the city more green and more social is of course secondary to that `stip aan de horizon'. Special thanks goes out to, April, Cilia, Giedo, Jan, Joep, Lisa, Louis, Marieke, Nynke, Pepijn O.~and Wouter.

...

All of you made me who I am and brought me to where I am, and I am immensely grateful for that.

